Price of metric universality in vector quantization is at most 0.11 bit

Fast computation of a matrix product $W^\top X$ is a workhorse of modern LLMs. To make their deployment more efficient, a popular approach is that of using a low-precision approximation $\widehat W$ in place of true $W$ (``weight-only quantization''). Information theory demonstrates that an optimal algorithm for reducing precision of $W$ depends on the (second order) statistics of $X$ and requires a careful alignment of vector quantization codebook with PCA directions of $X$ (a process known as ``waterfilling allocation''). Dependence of the codebook on statistics of $X$, however, is highly impractical. This paper proves that there exist a universal codebook that is simultaneously near-optimal for all possible statistics of $X$, in the sense of being at least as good as an $X$-adapted waterfilling codebook with rate reduced by 0.11 bit per dimension in the case when $W$ is Gaussian. Such universal codebook would be an ideal candidate for the low-precision storage format, a topic of active modern research, but alas the existence proof is non-constructive. Equivalently, our result shows existence of a net in $\mathbb{R}^n$ that is a nearly-optimal covering of a sphere simultaneously with respect to all Hilbert norms.

==> MutualInfo.tex <==
\section{Heuristic Mutual Information Proof of the RCRD Region}
\label{sec:MI}

One of the main challenges in our setup is that we must use the same codebook for describing $\hat{W}$, regardless of what $\Sigma_X$ is. In terms of random coding, this corresponds to drawing the $2^{nR}$ codewords iid using a distribution $P_{\hat{W}}$ that does not depend on $\Sigma_X$. 

In rate-distortion theory, one needs to find a coupling $P_{W\hat{W}}$ with marginals $P_W$ corresponding to the source distribution which is $\m{N}(0,I_n)$ in our setup, and $P_{\hat{W}}$ corresponding to the codewords distribution, with small mutual information and distortion. 

In this section, for any $T>0$ we provide a coupling between $P_W=\m{N}(0,I_n)$ and $P_{\hat{W}}=\m{N}(0,\tau^2 I_n)$ that attains
\begin{align}
I(W;\hat{W})&=\sum_{i=1}^n \frac{1}{2}\log \left(1+T\lambda_i \right)\\
\EE\|\Lambda^{1/2}U^\top (W-\hat{W})\|_2^2&=\sum_{i=1}^n \lambda_i \left(1-2\tau\sqrt{\frac{\lambda_iT}{1+\lambda_i T}} +\tau^2\right).
\end{align}
Substituting 
\begin{align}
\tau=    \frac{\sum_{i=1}^n \lambda_i\sqrt{\frac{\lambda_iT}{1+\lambda_i T}} }{\sum_{i=1}^n\lambda_i}
\end{align}
gives
\begin{align}
\frac{1}{n}I(W;\hat{W})= R_n^\rc(\Lambda, T),~~   \frac{1}{n}\EE\|\Lambda^{1/2}U^\top (W-\hat{W})\|_2^2=D_n^\rc(\Lambda, T)+\Delta,
\end{align}
for $\Delta>0$. \OrComm{It seems like finding a coupling with $\Delta=0$ is impossible, because the reconstruction distribution $P_{\hat{W}}=\m{N}(0,\tau^2 I)$ is not simultaneously optimal for all $\Sigma_X$. Consequently, the actual ``codeword success exponent'' is
$$-\log p_n=\min_{P_{Y|W}:\EE\|\Lambda^{1/2}U^\top (W-Y)\|_2^2\leq D}(P_{Y|W}\|\m{N}(0,\tau^2 I_n)|P_W)$$ which is greater than 
\begin{align*}
&\min_{P_{Y|W}:\EE\|\Lambda^{1/2}U^\top (W-Y)\|_2^2\leq D,P_Y=\m{N}(0,\tau^2 I_n)}(P_{Y|W}\|\m{N}(0,\tau^2 I_n)|P_W)\\
&=\min_{P_{Y|W}:\EE\|\Lambda^{1/2}U^\top (W-Y)\|_2^2\leq D,P_Y=\m{N}(0,\tau^2 I_n)}I(W;Y).    
\end{align*}
It is conceivable that among all couplings $P_{W\hat{W}}$ the one given below achieves the smallest possible worst-case $\Delta>0$. It might be useful for designing of practical schemes: the filters below can be incorporated into waterSIC.}

Recall that $\Sigma_X=U\Lambda U^\top$. For $T>0$, our coupling constructs $$\hat{W}=F(HW+T^{-1/2}Z),$$
where
\begin{itemize}
\item $W,Z\sim\m{N}(0,I_n)$, $W\indep Z$.
\item  $H=\Lambda^{1/2}U^\top$
\item $F=\tau U T^{1/2}\left(I+T\Lambda \right)^{-1/2}$
\end{itemize}
Let us verify that this indeed give the claimed properties. First, by the data processing inequality (DPI)
\begin{align}
I(W;\hat{W})\leq I(W;HW+T^{-1/2}Z)=\frac{1}{2}\log\frac{|H H^\top+T^{-1}I_n|}{|T^{-1}I_n|}=\sum_{i=1}^n\frac{1}{2}\log\left(1+T\lambda_i) \right) .   
\end{align}
where the first inequality holds with equality whenever $F$ us non-singular, i.e., whenever $\lambda_i>0$ for all $i$. It is clear that $\hat{W}$ is a zero-mean Gaussian vector. It's covariance is
\begin{align}
\EE[\hat{W}\hat{W}^\top]=F\EE\left[\left(HW+\frac{1}{\sqrt{T}}Z\right)\left(HW+\frac{1}{\sqrt{T}}Z\right)^\top \right]F^\top    =F\left[\Lambda+\frac{1}{T}I_n\right]F^\top=\tau^2 I_n.
\end{align}
It remains to compute the distortion. Denote $W'=U^\top W\sim\m{N}(0,I_n)$ and write
\begin{align}
e&=U^\top(W-\hat{W})=W'-U^\top FHW-U^\top F T^{-{1/2}}Z\\
&=W'-\tau (T\Lambda)^{1/2}(I+T\Lambda)^{-1/2}W'-\tau(I+T\Lambda)^{-1/2}Z.  
\end{align}
Consequently,
\begin{align}
D(\tau)&=\EE\|\Lambda^{1/2}e\|^2=\sum_{i=1} \lambda_i\left[\left(1-\tau\sqrt{\frac{\lambda_i T}{1+\lambda_i T}} \right)^2+\tau^2\frac{1}{1+\lambda_i T} \right]\nonumber\\
&=\sum_{i=1}\lambda_i\left(1-2\tau\sqrt{\frac{\lambda_i T}{1+\lambda_i T}} +\tau^2\right)   
\end{align}

==> typicalSetProb.tex <==
\section{Proof of Lemma~\ref{lem:Ptypical}}
\label{sec:typicalSetProb}

Let $A\diag\left(\frac{\lambda_1}{1+\lambda_1 T},\ldots,\frac{\lambda_n}{1+\lambda_n T}\right)$. Since $\frac{\lambda}{1+\lambda T}\leq \frac{1}{T}$ for all $\lambda>0$ we have that $\|A\|_{op}\leq\frac{1}{T}$ and $\|A\|_F^2\leq\frac{n}{T^2}$. By definition of $T=T(\Sigma_X,R)$ is satisfies
\begin{align}
R=\frac{1}{n}\sum_{i=1}^n \frac{1}{2}\log(1+\lambda_i T)\leq \frac{\log e}{2n}\sum_{i=1}^n\lambda_i T=\frac{\log e}{2}T,
\end{align}
since $\trace(\Sigma_X)=n$. Consequently, $\frac{1}{T}\leq \frac{\log 2}{2R}$, which implies
\begin{align}
\frac{1}{ \|A\|_F^2}\leq n\frac{\log^2 e}{4R^2} ,~~~~~~\frac{1}{\|A\|_{op}}\leq \frac{\log e}{2R}.
\end{align}
\nbyp{Wrong direction of inequalities?}
Let $\Wt=U^\top W\sim\m{N}(0,I_n)$. We have that
\begin{align}
\Pr&\left(\left|\sum_{i=1}^n\frac{\lambda_i}{1+\lambda_i T(\Sigma_X,R)} \left((U^\top W)^2_i-1\right) \right|  \leq n\cdot \frac{\eta}{3} \right)=\Pr\left(|\Wt^\top A \Wt-\trace{A}|\geq n\cdot\frac{\eta}{3} \right)\nonumber\\
&\leq 2\exp\left\{-c~\min\left(n\frac{\eta^2 \log^2 e}{9\cdot 4R^2 K^4},n\frac{\eta\log e}{3\cdot 2R K^2} \right)\right\},
\end{align}
where the last inequality holds for some universal constants $c,K>0$ and is due to Proposition~\ref{prop:hanson_wright}. In addition, by the union bound we have
\begin{align}
\Pr(\|\Wt\|_{\infty}\geq t)\leq n \Pr(|\Wt_1|\geq t)\leq n e^{-\frac{t^2}{2}},
\end{align}
which implies that
\begin{align}
\Pr\left( \|\Wt\|_{\infty}\geq n^{1/5}\right)  \leq c_1 e^{-c_2 n^{3/10}},
\end{align}
for some universal constants $c_3,c_4$. Using the union bound, it follows that there exist universal constants $c_1>0$ and $c_2=c_2(\eta,R)>0$ for which the claim holds.


==> worst_case_gap.tex <==
\section{Worst-Case Gap Between Waterfilling and Random Coding: Theorem~\ref{thm:worst_case} and Lemma~\ref{lem:worst_case_D_lim}}\label{sec:worst_case}

Recall that for $\Lambda = \diag\paren{\lambda_1,\dots,\lambda_n} \succeq 0$ with $ \trace (\Lambda) = n$, the random-coding rate-distortion is given by a parametric relationship 
\begin{equation}\label{eq:rc_rd_worst}
    \Drc(\Lambda, T) = \frac 1 n \sum_{i=1}^n \frac{\lambda_i}{1+\lambda_i T}\qquad \Rrc(\Lambda, T) = \frac 1 {2 n}\sum_{i=1}^n \log(1+\lambda_i T)\,,\tag{RDRC}
\end{equation}
and the waterfilling rate-distortion by 
\begin{equation}\label{eq:wf_rd_worst}
    \Dwf(\Lambda, t) = \frac{1}{n}\sum_{i=1}^n \min\sset{\lambda_i,t}\qquad \Rwf(\Lambda, t) = \frac 1 {2n} \sum_{i=1}^n \max\sset{0, \log (\lambda_i/t)}\,.\tag{RDWF}
\end{equation}
Throughout, $\log$ denotes the base-2 logarithm, and $\ln$ denotes the natural logarithm. The goal of this section is to quantify, at a fixed target distortion $\Dstar$, the rate overhead of our universal codebook, whose rate-distortion is given in Eq.~\eqref{eq:rc_rd_worst}, compared to the $\Sigma_X$-fine-tuned optimal codebook, whose rate-distortion is given in Eq.~\eqref{eq:wf_rd_worst}.

Denote\footnote{All of the $\Drc, \Dwf, \Rrc, \Rwf$ are monotone in $T, t$.} the implicit functions $\Trc(\Lambda, \Dstar) = T^\star$ s.t. $\Drc(\Lambda, T^\star) = \Dstar$ and $\twf(\Lambda, \Dstar) = t^\star$ s.t. $\Dwf(\Lambda, t^\star) = \Dstar$. Denote 
\begin{equation*}\label{eq:rrrc_rrwf}
    \RRrc(\Lambda, \Dstar) = \Rrc(\Lambda, \Trc(\Lambda, \Dstar)) \qquad\text{and}\qquad \RRwf(\Lambda, \Dstar) = \Rwf(\Lambda, \twf(\Lambda, \Dstar))\,.
\end{equation*}
In this notation, the rate overhead incurred by our universal codebook is 
$$
\sup_{\Lambda} \sset{ \RRrc(\Lambda, \Dstar) - \RRwf(\Lambda, \Dstar)}\,,
$$
where the supremum is over $\Lambda = \diag(\lambda_1,\dots,\lambda_n)\succeq 0$ with $\trace(\Lambda) = n$. We establish the claimed $0.11$bit rate gap bound in two complementary ways. First, Theorem~\ref{thm:worst_case} shows that for any fixed $\Dstar \in \sqb{\delta, 1 - \delta}$ with $\delta = 0.005$,
$$
\sup_{\Lambda} \sset{ \RRrc(\Lambda, \Dstar) - \RRwf(\Lambda, \Dstar)} \leq 0.11\,.
$$
To prove Theorem~\ref{thm:worst_case} in Sec.~\ref{subsec:worst_case_proof}, we first verify that the maximum is attained at\footnote{After reducing to an optimization-friendly version, see Claim~\ref{claim:interior}.} $\Lambda^\star$ which contains at most $5$ distinct eigenvalues (Claims~\ref{claim:lower_tail}, \ref{claim:3_vals}). We then numerically verify the worst-case $0.11$ bit upper bound for such spectrums (Claim~\ref{claim:numerical}). 

Second, Lemma~\ref{lem:worst_case_D_lim} controls the rate gap in the small-distortion regime $\Dstar \to 0$ and shows
$$
\limsup_{\Dstar \to 0} \paren{\sup_{\Lambda} \sset{ \RRrc(\Lambda, \Dstar) - \RRwf(\Lambda, \Dstar)}} \leq 0.11\,.
$$
This is proved in Sec.~\ref{subsec:worst_case_D_lim_proof} by passing to a limiting measure over rescaled spectra.

\subsection{Proof of Theorem~\ref{thm:worst_case}}\label{subsec:worst_case_proof}

\begin{mythm}{\ref{thm:worst_case}}\textnormal{\textbf{(Worst-Case Gap Between Waterfilling and Random Coding)}}
    For any fixed $\Dstar \in \sqb{\delta, 1 - \delta}$ with $\delta = 0.005$, assuming the numerical result in Claim~\ref{claim:numerical},
    $$
    \sup_{\Lambda} \sset{ \RRrc(\Lambda, \Dstar) - \RRwf(\Lambda, \Dstar)} \leq 0.11\,,
    $$
    where the supremum is over $\Lambda = \diag(\lambda_1,\dots,\lambda_n)\succeq 0$ with $\trace(\Lambda) = n$.
\end{mythm}
\begin{proof}(of Theorem~\ref{thm:worst_case})
    In this proof we fix one value $\Dstar \in \sqb{\delta, 1- \delta}$ and for convenience denote 
    $$
    \RRrc(\Lambda) = \RRrc(\Lambda, \Dstar)\qquad \text{and}\qquad \RRwf(\Lambda) = \RRwf(\Lambda, \Dstar)\,.
    $$
    Similarly, we write 
    $$
    \Trc(\Lambda) = \Trc(\Lambda, \Dstar) \qquad\text{and}\qquad \twf(\Lambda) = \twf(\Lambda, \Dstar)\,.
    $$
    First, we show that in our optimization it is sufficient to consider $\Lambda=\diag(\lambda_1,\dots,\lambda_n)$ such that $\min_i |\twf(\Lambda) - \lambda_i|$ is bounded away from $0$, i.e. none of the eigenvalues are close to the waterfilling level $\twf(\Lambda)$:
    \begin{claim}\label{claim:interior} Fix $\Dstar \in \sqb{\delta, 1- \delta}$. For any $\eps \in (0, \Dstar)$ and $f_n = (\Dstar-\eps) / (2n)$,  
        $$
        \sup_{\Lambda} \sset{ \RRrc(\Lambda) - \RRwf(\Lambda)} \leq \sup_{\substack{\Lambda: \min_i |\lambda_i - \twf(\Lambda, D)|\\ \geq \eps f_n}} \sset{ \RRrc(\Lambda, D) - \RRwf(\Lambda, D) \ \b|\ D \in \sqb{\Dstar-\eps, \Dstar} } + \eps\,,
        $$
        where we only consider $\Lambda = \diag(\lambda_1,\dots,\lambda_n)\succeq 0$ with $\trace(\Lambda) = n$.
    \end{claim}
    For $\eps > 0$ and $f_n = \Dstar / (2n)$ we now focus on the restricted optimization problem 
\begin{equation}\label{eq:restricted_opt_all_k}
        \sup_{\substack{\Lambda: \min_i |\lambda_i - \twf(\Lambda)|\\ \geq \eps f_n}} \sset{ \RRrc(\Lambda) - \RRwf(\Lambda)}\,.
    \end{equation}
    For any $\Lambda$ we define
    \begin{align*}
        \text{active set:} &\quad \calA_\Lambda = \sset{i\in \sqb{n}:\, \lambda_i > \twf(\Lambda)}\,,\\
        \text{inactive set:} &\quad \calI_\Lambda = \sset{i\in \sqb{n}:\, \lambda_i \leq \twf(\Lambda)}\,.
    \end{align*}
    We now split our optimization into $n+1$ case based on the size of active set $k \coloneq |\calA_\Lambda|$. For a fixed active set of size $k$, WLOG $\calA = \sqb{k}$, consider
    \begin{equation}\label{eq:k_opt_argmax}
       \sup_{\substack{\Lambda: \min_i |\lambda_i - \twf(\Lambda)|\\ \geq \eps f_n, \calA = \sqb{k}}} \sset{ \RRrc(\Lambda) - \RRwf(\Lambda) }\,.
    \end{equation}
    Denote $G(\Lambda) = \RRrc(\Lambda) - \RRwf(\Lambda)$ and rewrite the optimization problem in Eq.~\eqref{eq:k_opt_argmax} as follows:
    \begin{align}
        \inf_{\Lambda} &- G(\Lambda) \quad \qquad\text{subject to}\tag{obj}\label{eq:obj}\\
        \lambda_i &\geq \twf(\Lambda) + \eps f_n \qquad\text{ for all }i\in\sqb{k}\tag{active}\label{eq:active}\\
        0 &\leq \lambda_i \leq \twf(\Lambda) - \eps f_n \qquad\text{ for all }i > k\tag{inactive}\label{eq:inactive}\\
        \sum_i \lambda_i &= n\tag{trace}\label{eq:trace}\,.
    \end{align}
    First, for fixed $\calA$ as above and $t \coloneq \twf(\Lambda), T\coloneq \Trc(\Lambda)$, 
    $$
    n\Dstar = n\Dwf(\Lambda, t) = \sum_{i=k+1}^n \lambda_i + kt \quad\text{and}\quad n\RRwf(\Lambda) = n\Rwf(\Lambda, t) = \frac12 \sum_{i=1}^k \log(\lambda_i / t)\,, \quad\text{so}
    $$
    $$2n G(\Lambda) = 2n \RRrc(\Lambda) - 2n \RRwf(\Lambda) = \sum_{i=1}^n \log(1+\lambda_i T) -  \sum_{i=1}^k \log (\lambda_i) + k\log t\,.$$
    Therefore, the objective in Eq.~\eqref{eq:obj} is continuous and, from the trivial bounds on $t, T$\footnote{From Eq.~\eqref{eq:inactive} and $\Dstar < 1$, $0\leq t \leq \max_i \lambda_i \leq n$. From $\Dstar \leq 1 -\delta$, $T \geq g(\delta) > 0$ and from $\Dstar \geq \delta$, $1+nT \leq n/\delta$.}, the feasible set is compact, and therefore, the optimum value is attained at some \begin{equation}\label{eq:lambda_k_star}
        \Lambda_k^\star \coloneq \argmax_{\substack{\Lambda: \min_i |\lambda_i - \twf(\Lambda)|\\ \geq \eps f_n, \calA = \sqb{k}}} \sset{ \RRrc(\Lambda) - \RRwf(\Lambda) }\,.
    \end{equation}
    \begin{claim}[Inactive Set Equalizes]\label{claim:lower_tail}
        In the setting above, $\Lambda_k^\star = \diag(\lambda_1^\star, \dots, \lambda_n^\star)$ from Eq.~\eqref{eq:lambda_k_star} satisfies 
        $$ \lambda_{k+1}^\star = \dots \lambda_n^\star\,.$$
    \end{claim}

    \begin{claim}[Active Set Has at Most $4$ Distinct Values]\label{claim:3_vals}
        In the setting above, $\Lambda_k^\star = \diag(\lambda_1^\star, \dots, \lambda_n^\star)$ from Eq.~\eqref{eq:lambda_k_star} has at most $5$ distinct eigenvalues.
    \end{claim}

    Finally, we numerically verify that among $\Lambda$ with at most $5$ distinct values, the objective function does not exceed $0.11$, which yields, combined with previous claims, the statement of the theorem.

    \begin{claim}[Worst-Case Gap is at Most $0.11$, Numerical]\label{claim:numerical}
        For $\Dstar \in \sqb{\delta, 1 -\delta}$ for $\delta = 0.005$, 
        $$
        \sup_{\substack{\Lambda: \b|\sset{\lambda_i}\b| \leq 5,\\ \min_i |\lambda_i - \twf(\Lambda)| \geq \eps f_n}} \sset{ \RRrc(\Lambda) - \RRwf(\Lambda) } < 0.11\,,
        $$
        where the optimization is over $\Lambda = \diag(\lambda_1,\dots, \lambda_n) \succeq 0$ with $\trace(\Lambda) = n$.
    \end{claim}

    
    


\end{proof}


\begin{proof}(of Claim~\ref{claim:interior})
        Fix any $\Lambda = \diag(\lambda_1,\dots,\lambda_n)\succeq 0$ with $\trace(\Lambda) = n$ and let $t = t(\Lambda, \Dstar)$. Consider $$t' = \argmin_{t' \leq t: \min_i |\lambda_i - t'| \geq \eps f_n}|t'- t|\,.$$
        First, with the definitions above, $t - 2\eps n f_n \leq t' \leq  t$, since there are total of $n$ eigenvalues. Moreover, 
        $$
        \underbrace{\Dwf(\Lambda, t)}_{\Dstar} - 2\eps n f_n \leq \underbrace{\Dwf(\Lambda, t')}_{\coloneq D} \leq \underbrace{\Dwf(\Lambda, t)}_{\Dstar} \,.
        $$
        Let $T' = T(\Lambda, D)$: by monotonicity, $T' \geq T=T(\Lambda, \Dstar)$. Then, $$\Rrc(\Lambda, T') \geq \underbrace{\Rrc(\Lambda, T)}_{\RRrc(\Lambda)}\,.$$
        Since $D \leq t'$,
        $$
        \Rwf(\Lambda, t') - \underbrace{\Rwf(\Lambda, t)}_{\RRwf(\Lambda)}  \leq \frac 12 \log (t/t') \leq \frac{t-t'}{2t'} \leq \frac{t'-t}{2D} \leq \eps n f_n /(\Dstar - 2\eps n f_n)\,.
        $$
        Taking $f_n = (\Dstar-\eps) / (2n)$, we obtain the claim.
    \end{proof}


\begin{proof}(of Claim~\ref{claim:lower_tail})
    We prove that the objective $G(\Lambda)$ is Schur-concave in $\lambda_{k+1},\dots,\lambda_{n}$ (the eigenvalues from the inactive set $\calI_{\Lambda}$. For this, we compute:
    \begin{align*}
        \frac{\partial \twf(\Lambda)}{\partial \lambda_i} &= -\frac{\frac{\partial \Dwf(\Lambda, t)}{\partial \lambda_i}}{\frac{\partial \Dwf(\Lambda, t)}{\partial t}} = - \frac{ 1 }{k} &\text{for }i> k\,,\\
        \frac{\partial \Trc(\Lambda)}{\partial \lambda_i} &= -\frac{\frac{\partial \Drc(\Lambda, T)}{\partial \lambda_i}}{\frac{\partial \Drc(\Lambda, T)}{\partial T}} = \frac{ \frac 1 {(1+\lambda_i T)^2} }{\sum_{j=1}^n \frac{\lambda_j^2}{(1+\lambda_j T)^2}} &\text{for all }i\in \sqb{n}\,.
    \end{align*}
    We plug this into 
    \begin{align*}
        \frac{\partial 2n\RRwf(\Lambda)}{\partial \lambda_i} &= 0 - k \frac{1}{t\ln 2} \cdot \B(- 1/ k\B) = \frac 1 {t\ln 2} &\text{for }i>k\,,\\
        \frac{\partial 2n\RRrc(\Lambda)}{\partial \lambda_i} &= \frac T {(1+\lambda_i T)\ln 2} + \B(\sum_{j=1}^n \frac {\lambda_j} {(1+\lambda_j T)\ln 2}\B) \cdot \frac{ \frac 1 {(1+\lambda_i T)^2} }{\sum_{j=1}^n \frac{\lambda_j^2}{(1+\lambda_j T)^2}} &\text{for all }i\in\sqb{n}\,.
    \end{align*}
    Finally, $\frac{\partial 2n G(\Lambda)}{\partial \lambda_i} = \frac{\partial 2n\RRrc(\Lambda)}{\partial \lambda_i} - \frac{\partial 2n\RRwf(\Lambda)}{\partial \lambda_i}$. From expressions above, for any $\Lambda$ and $i > k$, 
    $$
    (\lambda_i - \lambda_j) \B( \frac{\partial 2n G(\Lambda)}{\partial \lambda_i} - \frac{\partial 2n G(\Lambda)}{\partial \lambda_j} \B) \leq 0\,,
    $$
    which yields the desired statement.

\end{proof}

\begin{proof}(of Claim~\ref{claim:3_vals})
    For the optimization problem in Eq.~\eqref{eq:obj}, we first verify that the optimizer $\Lambda_k^\star$ either immediately satisfies Claim~\ref{claim:3_vals} or admits the LICQ conditions; we conclude that $\Lambda_k^\star$ satisfies the KKT conditions, from which we derive Claim~\ref{claim:3_vals}.
    
    \paragraph{Step I: LICQ.} Assume that the optimizer $\Lambda^\star_k$ has at least $4$ distinct values. We have
    $$
    \frac{\partial \twf(\Lambda)}{ \partial \lambda_i} = \begin{cases}
        -1/k, & i > k\\
        0, &\text{otherwise}.
    \end{cases}
    $$
    Denoting the equality constraint $h(\Lambda) = \sum_i \lambda_i - n$ and inequality constraints $g_i(\Lambda) = \begin{cases}
        -\lambda_i + \twf(\Lambda) + \eps f_n, & i\leq k\\
        \lambda_i - \twf(\Lambda) + \eps f_n, & i > k
    \end{cases}$ and $f_i(\Lambda) = -\lambda_i$ for $i > k$, we compute
    \begin{align*}
        \nabla h &= \paren{ 1,\dots,1}\,,&\\
        \nabla g_i &= (-1)^{\I_{i\leq k}}(e_{i} + (0, \dots, 0, 1/k,\dots,1/k)) &\text{for all }i\,,\\
        \nabla f_i &= - e_i &\text{for } i>k\,.
    \end{align*}

    Consider a minimal linearly dependent set $\mathcal{S}$ of $\nabla h$ and the gradients of the active constraints $g_i, f_i$. Recall that from Claim~\ref{claim:lower_tail}, the optimizer $\Lambda^\star$ satisfies $\lambda_{k+1}^\star = \dots = \lambda_n^{\star}$.
    \begin{itemize}
        \item Case 1: $\nabla h \not\in \mathcal S$. Then for all $i \leq k$, $\nabla g_i \not \in \mathcal S$. Since $\eps f_n = \eps \Dstar / (2n) < \Dstar \leq t$, for each $i > k$, at most one of $\nabla g_i$ or $\nabla f_i$ is active. Then either there are at most $3$ distinct values in $\Lambda^\star$ (which would lead to contradiction), or, for at least one $i > k$ none of the $g_i, f_i$ are active ($\nabla g_i, \nabla f_i \not\in \mathcal S$), in which case $\mathcal S$ is linearly independent. 
        \item Case 2: $\nabla h \in \mathcal S$. Then, for each $i\leq k$, $g_i \in \mathcal S$, and therefore $\Lambda^\star$ has at most two distinct values, contradiction.
    \end{itemize}
    We conclude that, in the case where $\Lambda^\star_k$ has more than $3$ distinct eigenvalues, LICQ holds.
    
    \paragraph{Step II: KKT.} Assume that the optimizer $\Lambda^\star_k$ has at least $4$ distinct values: by Step I, $\Lambda^\star_k$ satisfies the KKT conditions. For $u \in \R^{2n-k}, v \in \R$ , denote 
    \begin{equation*}
        L(\Lambda, u , v) \triangleq - G(\Lambda) + \sum_{i=1}^n u_i g_i(\Lambda) + \sum_{i=k+1}^n u_{n-k+i} f_i(\Lambda) + v h(\Lambda)\,.
    \end{equation*}
    For $i \leq k$, 
    \begin{align*}
        \frac{\partial \twf(\Lambda)}{\partial \lambda_i} &= -\frac{\frac{\partial \Dwf(\Lambda, t)}{\partial \lambda_i}}{\frac{\partial \Dwf(\Lambda, t)}{\partial t}} = 0\,.
    \end{align*}
    We plug this into $
        \frac{\partial 2n\RRwf(\Lambda)}{\partial \lambda_i} = \frac 1 {\lambda_i \ln 2}$ and recall that for all $i\in\sqb{n}$, 
        \begin{align*}
        \frac{\partial 2n\RRrc(\Lambda)}{\partial \lambda_i} = \frac T {(1+\lambda_i T)\ln 2} + \underbrace{\B(\sum_{j=1}^n \frac {\lambda_j} {(1+\lambda_j T)\ln 2}\B) \cdot \frac{ \frac 1 {(1+\lambda_i T)^2} }{\sum_{j=1}^n \frac{\lambda_j^2}{(1+\lambda_j T)^2}}}_{\coloneq A_\Lambda \cdot \frac{1}{(1+\lambda_i T)^2 \ln 2}}\,.
    \end{align*}
    From the complementary slackness, for all $i\geq k$ for which $g_i(\Lambda) = -\lambda_i + \twf(\Lambda) + \eps f_n < 0$, we have 
    \begin{align*}
        \frac{\partial G(\Lambda)}{\partial \lambda_i} = \frac{\partial \RRrc(\Lambda)}{\partial \lambda_i} - \frac{\partial \RRwf(\Lambda)}{\partial \lambda_i} = v\,,
    \end{align*}
    which we rewrite as 
    $$
    \frac{T}{1+\lambda_i T} + \frac{A_\Lambda}{(1+\lambda_i T)^2} - \frac 1 {\lambda_i} = 2n v \ln 2\,. 
    $$
    We conclude that there are to most $3$ distinct values that eigenvalues $\lambda_i \neq \twf(\Lambda) + \eps f_n$ can take for $i \leq k$, concluding the proof. 
\end{proof}

\subsection{Proof of Lemma~\ref{lem:worst_case_D_lim}}\label{subsec:worst_case_D_lim_proof}

\begin{mylem}{\ref{lem:worst_case_D_lim}}\textnormal{(Finite-dimensional small-distortion 0.11 bit bound)}
    $$
        \limsup_{\Dstar \to 0} \paren{\sup_{\Lambda} \sset{ \RRrc(\Lambda, \Dstar) - \RRwf(\Lambda, \Dstar)}} \leq 0.11\,,
    $$
    where the supremum is over $\Lambda = \diag(\lambda_1,\dots,\lambda_n)\succeq 0$ with $\trace(\Lambda) = n$.
\end{mylem}

Lemma~\ref{lem:worst_case_D_lim} follows immediately from a more general version of the same statement in Lemma~\ref{lem:worst_case_D_lim_measure}. Let $\mathcal{P}([0,\infty))$ denote the space of Borel probability measures on $[0,\infty)$, and define
$$
\mathcal{P}_1([0,\infty)) = \sset{\lambda \in \mathcal{P}([0,\infty)): \int x d\lambda(x) = 1}\,.
$$
We extend the finite-dimension rate-distortion curves in Eq.~\eqref{eq:rc_rd_worst} and \eqref{eq:wf_rd_worst} as follows: for $\mu \in \mathcal{P}_1([0,\infty))$, let
$$
\Drc(\mu,T)
=
\int_0^\infty \frac{x}{1+xT}d\mu(x),
\qquad
\Rrc(\mu,T)
=
\frac12\int_0^\infty \log(1+xT)d\mu(x),
$$
and
$$
\Dwf(\mu,t)
=
\int_0^\infty \min\sset{x,t}d\mu(x),
\qquad
\Rwf(\mu,t)
=
\frac12\int_0^\infty \max\sset{0,\log(x/t)}d\mu(x).
$$
Similarly to above, for each $\Dstar\in(0,1)$, let $\Trc(\mu,\Dstar)$ and $\twf(\mu,\Dstar)$ be defined by
$
\Drc(\mu,\Trc(\mu,\Dstar))=\Dstar$ and $\Dwf(\mu,\twf(\mu,\Dstar))=\Dstar,
$
and set
$$
\RRrc(\mu,\Dstar)
=
\Rrc(\mu,\Trc(\mu,\Dstar)),
\qquad
\RRwf(\mu,\Dstar)
=
\Rwf(\mu,\twf(\mu,\Dstar)).
$$

\begin{lemma}[Small-distortion 0.11 bit bound]\label{lem:worst_case_D_lim_measure}
    $$
    \limsup_{\Dstar \to 0} \paren{\sup_{\mu} \sset{ \RRrc(\mu, \Dstar) - \RRwf(\mu, \Dstar)}} \leq 0.11\,,
    $$
    where the supremum is over probability measures $\mu \in \mathcal{P}_1([0, \infty))$.
\end{lemma}
\begin{proof}
The result is obtained by first passing to a limiting measure. Denote the rate-gap
$$
\Delta (\mu, \Dstar) = \frac 12 \int r_{\Trc(\mu, \Dstar), \twf(\mu, \Dstar)}(x) d \mu(x)\,, \qquad r_{T, t}(x) = \begin{cases}
    \log(1+xT) &\text{if } x \leq t\\
    \log\paren{\frac{1+xT}{x/t}} &\text{if } x > t\,.
\end{cases}
$$
It will be convenient to consider the following rescaling:
$$
\mut \coloneq (x \to x/\Dstar)_{\sharp \mu}\,, \qquad \ttilde = \twf(\mu, \Dstar)/\Dstar\,, \qquad \Ttilde = \Trc(\mu, \Dstar)\cdot\Dstar\,.
$$
With this rescaling, the distortion definitions and the expression for the rate gap become
\begin{equation}\label{eq:dist_reparam}
1 = \int \frac{x}{1+x \Ttilde} d \mut(x) = \int \min\sset{x,\ttilde} d\mut(x)\qquad \text{and} \qquad 2 \Delta(\mu, \Dstar) \coloneq \int r_{\Ttilde, \ttilde}(x) d\mut(x)\,.
\end{equation}
Note that $\int x d \mut (x) = (\Dstar)^{-1}$. 


Let $\kappa = \int_{\ttilde}^{+\infty} d\mut(x)$ be the mass $\mut$ puts to the waterfilling-active modes. Expanding $\int \min\sset{x,\ttilde} d\mut(x) = \int_{0}^{\ttilde}x d\mut(x) + \kappa \ttilde$, from Eq.~\eqref{eq:dist_reparam} we conclude 
   $$
   \ttilde \geq 1\,, \qquad \Ttilde \leq 1\,, \qquad \ttilde \Ttilde \leq 1\,,
   $$
   where the last inequality is derived as follows:
   \begin{align*}
       1 = \int \frac{x}{1+x \Ttilde} d \mut(x) \leq \int_{0}^{\ttilde} x d \mut(x) + \frac \kappa \Ttilde = (1 - \kappa \ttilde) + \frac \kappa \Ttilde = 1 + \kappa \paren{-\ttilde + \frac 1 \Ttilde}\,.
   \end{align*}
   We now obtain bounds on $\Delta(\mu, \Dstar)$ in terms of $\ttilde, \Ttilde$:
   \begin{align*}
       \Delta(\mu, \Dstar) &= \underbrace{\frac 1 {2} \int_0^{\ttilde} \log(1+x \Ttilde) d \mut(x)}_{\mathsf{I}} +  \underbrace{\frac 1 {2} \int_{\ttilde}^{+\infty} \log \paren{\frac{1+x \Ttilde}{x / \ttilde}}d\mut(x)}_{\mathsf{II}}\,.
   \end{align*}
   From $\int \min \sset{x, \ttilde} d\mut(x) = 1$ and $\log(1+x) \leq x / \ln 2$, we bound 
   $\mathsf{I} \leq \frac {(1-\kappa)\Ttilde} {2\ln 2}$. To bound $\mathsf{II}$, notice that for $x \geq \ttilde$, $\log \paren{\frac{1+x\Ttilde}{x / \ttilde}} = \log (\ttilde\Ttilde + \ttilde /x) \leq \log(\ttilde\Ttilde + 1) \leq \ttilde \Ttilde /\ln 2$, so overall, 
   \begin{equation}\label{eq:gap_bound_tT}
   \mathsf{I} + \mathsf{II} \leq \frac {(1-\kappa)\Ttilde} {2\ln 2} + \frac{\kappa\ttilde \Ttilde}{2\ln 2}  \leq \frac {\Ttilde} {2\ln 2} + \frac{\Ttilde}{2\ln 2} = \frac {\Ttilde} {\ln 2} \leq \frac 1 {\ttilde \ln2}\,,
   \end{equation}
   where the last inequality used previously derived $\ttilde\Ttilde \leq 1$. Denote 
   $
    \Delta^\star \triangleq \limsup_{\Dstar \to 0} \paren{\sup_{\mu} \Delta(\mu, \Dstar)}\,.
    $
   Consider any sequence of spectra $\mu\up j$ and corresponding $D\up j \to 0$, such that
   $$
    \lim_{j \to \infty} \Delta(\mu \up j, D\up j) = \Delta^\star_\kappa\,.
    $$
    If $\limsup_{j\to\infty} \ttilde\up j = \infty$ or $\liminf_{j\to\infty} \Ttilde\up j = 0$, the bound in Eq.~\eqref{eq:gap_bound_tT} yields the lemma. Therefore, we can assume that (after truncating the sequence) that $\ttilde\up j \in [1, \ttilde\up 0]$ and $\Ttilde\up j \in [ \Ttilde\up 0, 1]$. Passing to a further subsequence, we may assume the weak convergence (in the compactification $[0,\infty]$) $$ \mut \up j \Rightarrow \mut \in \mathcal{P}([0,\infty])$$ and 
    $$
    \ttilde\up j \to \ttilde \in [1, \ttilde\up 0]\,, \qquad \Ttilde\up j \to \Ttilde \in [ \Ttilde\up 0, 1]\,, \qquad \kappa\up j \to \kappa \in [0,1]\,.
    $$
    Moreover, since on the compact set $[0, +\infty] \times [\Ttilde \up 0, 1] \times [1, \ttilde\up 0]$, the functions $\frac{x}{1+x \Ttilde}$, $\min\sset{x, \ttilde}$, and $r_{\Ttilde, \ttilde}(x)$ are continuous, the limiting measure satisfies the distortion constraints in Eq.~\eqref{eq:dist_reparam} and $\Delta(\mut) \triangleq \frac12 \int r_{\Ttilde, \ttilde}(x) d\mut(x) = \Delta^\star$ (with the natural extensions to $[0, +\infty]$ for the functions above). We will now optimize the limiting measure in a way that still satisfies the distortion constraints, while nondecreasing the rate gap. 

    First, we optimize the ``active" modes of $\mut$, i.e., the values $\geq \ttilde$. Recall the contribution to the rate gap is $$
    \frac 1 {2} \int_{\ttilde}^{+\infty} \log \paren{\frac{1+x \Ttilde}{x / \ttilde}}d\mut(x) = \frac 1 {2} \int_{\ttilde}^{+\infty} \log \paren{\ttilde \cdot \paren{\frac{x}{1+x \Ttilde}}^{-1}}d\mut(x)\,,
    $$
    where from Eq.~\eqref{eq:dist_reparam}, $\int_{\ttilde}^{\infty}\frac {x}{1+x \Ttilde} d\mut(x) = 1 - \int_{0}^{\ttilde}\frac {x}{1+x \Ttilde} d\mut(x)$. Note that for $x \geq \ttilde$, $\frac {x}{1+x \Ttilde} \in \sqb{\frac {\ttilde}{1+\ttilde \Ttilde}, \frac 1 \Ttilde}$ and is a monotone function, so by convexity of $f(y) = \log (\ttilde y^{-1})$, setting $$\mut(x) \propto \theta \cdot \delta_{\ttilde}(x) + (1-\theta) \cdot \delta_{+\infty}(x)\qquad\text{for }x\geq \ttilde$$ for some $\theta \in [0,1]$ will nondecrease the rate-gap.


    Finally, by the argument analogous to that of Claim~\ref{claim:3_vals}, we can further equalize the lower tail for the spectrum, setting 
    $$
    \mut(x) \propto \theta \cdot \delta_{\mut_0}(x) \qquad\text{for }x\leq \ttilde\,.
    $$ 
    It follows that
    $$
    2\Delta^\star \leq 2\Delta_{\mut} \leq  \theta \log(1+\mut_0\Ttilde) + (1-\theta) \log (\ttilde \Ttilde)\,,
    $$
    for some parameter $\theta \in [0,1]$ and, from Eq.~\eqref{eq:dist_reparam},
    $$
    1 = \theta\mut_0 + (1-\theta)\ttilde = \frac{\theta\mut_0}{1+\mut_0\Ttilde} + \frac{1-\theta}{\Ttilde}\,.
    $$
    The case $\theta = 1$ is impossible for $\Ttilde > 0$, so we will focus on the $\theta \in [0, 1)$ case.
    We now further simplify this optimization problem to obtain the final $0.11$ bound. 
    
    From the first distortion constraint, we express $\ttilde = (1-\theta)^{-1} - \paren{(1-\theta)^{-1} - 1} \mut_0$. From the second distortion constraint, $\Ttilde = \frac{\theta\mut_0\Ttilde}{1+\mut_0\Ttilde} + 1-\theta$, Denoting $\alpha = \mut_0 \Ttilde$, we then simplify $\ttilde\Ttilde  = (1-\theta)^{-1}\Ttilde - \paren{(1-\theta)^{-1} - 1} \alpha$. Plugging into the rate-gap bound:
    \begin{align*}
        2\Delta^\star_\kappa &\leq \theta\log(1+\alpha) + (1-\theta) \log \paren{1 + \frac{\theta\alpha}{(1+\alpha)(1-\theta)} - \frac{\alpha\theta}{1-\theta}}\\
        &=\theta\log(1+\alpha) + (1-\theta) \log \paren{1 - \frac{\alpha^2 \theta}{(1+\alpha)(1-\theta)} }\,,
    \end{align*}
    where from the positivity of $\ttilde, \Ttilde$ we have $0 \leq \theta < \frac{1+\alpha}{1+\alpha+\alpha^2}$ and $0 \leq \alpha = \mut_0 \Ttilde \leq \ttilde \Ttilde \leq 1$. Denoting $\rho = \frac{\theta}{1-\theta}$ and differentiating with respect to $\alpha$ gives 
    \begin{align*}
        \ln 2 (1-\theta)^{-1}\frac{\partial (2\Delta^\star)}{\partial \alpha} &= \frac{\rho}{1+\alpha} - \frac{1}{1 - \frac{\alpha^2\rho}{1+\alpha}}\cdot \rho \cdot \frac{2\alpha + \alpha^2}{(1+\alpha)^2}\\
        &=\frac{\rho}{1+\alpha}\paren{1 - \frac{2\alpha+\alpha^2}{1+\alpha - \alpha^2 \rho}}\,.
    \end{align*}
    Setting this to $0$ yields $\rho = \frac{1-\alpha - \alpha^2}{\alpha^2}$. At the boundary points $\alpha \in \sset{0,1}$, the objective function is below the objective of the Lemma. Plugging into the objective, we derive a one-parameter function 
    \begin{align*}
        2\Delta^\star \leq \frac{1-\alpha - \alpha^2}{1-\alpha} \log(1+\alpha) + \frac{\alpha^2}{1-\alpha}\log\paren{1 - \frac{1-\alpha-\alpha^2}{1+\alpha}}\,.
    \end{align*}
    The maximum of this objective is achieved at $\alpha\approx 0.35$ and is $\approx 2\cdot 0.108 < 2\cdot 0.11$, which concludes the proof.
\end{proof}



